Causal Imputation via Synthetic Interventions

Consider the problem of determining the effect of a compound on a specific cell type. To answer this question, researchers traditionally need to run an experiment applying the drug of interest to that cell type. This approach is not scalable: given a large number of different actions (compounds) and a large number of different contexts (cell types), it is infeasible to run an experiment for every action-context pair. In such cases, one would ideally like to predict the outcome for every pair while only having to perform experiments on a small subset of pairs. This task, which we label "causal imputation", is a generalization of the causal transportability problem. To address this challenge, we extend the recently introduced synthetic interventions (SI) estimator to handle more general data sparsity patterns. We prove that, under a latent factor model, our estimator provides valid estimates for the causal imputation task. We motivate this model by establishing a connection to the linear structural causal model literature. Finally, we consider the prominent CMAP dataset in predicting the effects of compounds on gene expression across cell types. We find that our estimator outperforms standard baselines, thus confirming its utility in biological applications.

==> content/algorithm.tex <==
\section{Algorithm}\label{sec:synthetic-interventions}

We extend the SI estimator introduced in \cite{agarwal2020synthetic} to handle more general sparsity patterns, learn across actions rather than contexts, and utilize multiple data sources for model-learning. 
%, developed within the context of policy evaluation. 
%
%we start by describing the estimator for our setup, and then argue that it is guaranteed to satisfy a factor model under a linear structural causal model. 
%
%Under the factor model, as argued in \cite{agarwal2020synthetic}, SI provably recovers the underlying $\cX$ of interest. 
%\subsection{Extending the Synthetic Interventions Estimator} \label{sec:si_estimator}
%
To describe our estimator, consider any target context-action pair $(c,a) \notin \Omega$.
%
As a high-level summary, our adapted SI estimator imputes the counterfactual $\bx^{ca}$ by appropriately weighting the observations $\{\bx^{cj}: j \in \cA(c)\}$.
%
Towards learning the weights, let $\cC_{\train} = \cC(\cA(c) \cup \{a\})$ denote the collection of contexts for which $\{x^{ij}: i \in \cC_\train, j \in \cA(c) \cup \{a\}\}$ are observed.
%
We call $\cA(c)$ and $\cC_\train$ the \textit{donor actions} and \textit{training contexts}, respectively.
%
We formally define the estimation strategy for imputing $\bx^{ca}$ below. 

\begin{enumerate}
    \item Model learning via linear regression 
    \begin{enumerate} 
    \item Let 
    $\bx_\train = [\bx^{ij}: i \in \cC_\train, j \in \cA(c)] \in \bbR^{p|\cC_\train| \times |\cA(c)|}$,  $\by_\train = [\bx^{ia}: i \in \cC_\train] \in \bbR^{p|\cC_\train|}$. 
    
    \item Define $\widehat{\beta} = \bx_\train^{\dagger} \by_\train \in \bbR^{|\cA(c)|}$,
    where $\bx_\train^{\dagger}$ denotes the pseudoinverse of $\bx_\train$. 
    \end{enumerate} 
    
    \item Counterfactual predictions
    \begin{enumerate} 
    \item Let $\bx_\test = [\bx^{cj}: j \in \cA(c)] \in \bbR^{p \times |\cA(c)|}$. 
    
    \item Define 
    $\widehat{\bx}^{ca} = \bx_\test \widehat{\beta}$. 
    \end{enumerate} 
\end{enumerate}

{\bf Comparisons with original SI estimator.} 
We note that the standard SI estimator is applied towards weighting $\{\bx^{ia}: i \in \cC(a)\}$ instead, i.e., the original SI estimator re-scales contexts rather than actions.
%
To carry out the standard approach, we follow the estimation strategy laid out above with $\cA_\train = \cA(\cC(a) \cup \{c\})$ and $\cC(a)$ replacing $\cC_\train$ and $\cA(c)$, respectively. Similarly, we call $\cC(a)$ the \textit{donor contexts} and $\cA_\train$ the \textit{training actions}.
%
We visualize both variants of the estimator and the associated terminology in \rref{app:method-visual}. 


\new{
%\textbf{Difference from the original SI estimator.} 
Notably, in the original SI framework, each context (unit) is seen under at most two actions: the control action during the pre-intervention period, and either a single other action or continued control action during the post-intervention period.
%
Thus, the \textit{only} weighting that can be learned is over contexts---there is no way to learn a weighting over actions.
%
This is a major limitation. 
As we will see in \rref{sec:empirical}, a weighting over contexts performs poorly for the task of causal imputation in the CMAP dataset. 
%
Furthermore, in this original setting, the context weights are learned using data from only a single action: the control action. Thus, $|\cA_\train| = 1$. Because our work allows for greater data flexibility, we may learn context weights from \textit{multiple} actions (or action weights from \textit{multiple} contexts, depending on the problem). This increase in training data allows the weights to be estimated more accurately. 
}

\new{\subsection{Practical Considerations}}

{\bf Using both estimators in tandem.}
The two estimators described above -- weighting actions and weighting contexts -- can be used in a complementary fashion.
%
For instance, say we apply the weighting actions estimator first. 
%
Then, the imputed values can increase the set of donor actions, which should lead to better outcomes when applying the weighting contexts estimator.
%
An analogous argument can be made when the weighting contexts estimator is applied first. 
%
This suggests a composite algorithm that iteratively applies each approach until the imputed tensor converges to a desired threshold. 
%
However, one drawback of this approach is that the estimator is computationally more demanding. 
% 
As such, formally motivating and analyzing such an algorithm remains to be interesting future work. 


{\bf Handling noise and sparsity.}
%
In many experimental settings, we may have measurement error and/or missing entries. 
%
In this case, \citet{agarwal2020synthetic} proposed first applying matrix estimation, i.e., $\ME: \bbR^{n \times p} \to \bbR^{n \times p}$ with $n$ denoting the size of donor contexts or actions, to $\bx_\train$ and $\bx_\test$ to ``de-noise'' the observations and fill in missing values. 
%
Popular $\ME$ methods include nuclear norm minimization and singular value thresholding, as analyzed by \citet{agarwal2020synthetic}. 

% \subsection{Robustness Checks}\label{sec:robustness_checks}
% %
% Below, we provide some robustness checks of when to use the SI estimator in practice.
% %
% We focus on the SI estimator that learns across actions, but analogous statements hold when SI learns across contexts.

\textbf{Arbitrary sets of donor actions.}
In the estimation strategy that we have described, we have assumed that our estimator will be a linear combination of \textit{all} actions $\cA(c)$ which are available for context $c$. In turn, this restricts the set of training contexts to only those contexts for which each of these actions, along with the target action, is measured, i.e., $\cC_\train = \cC(\cA(c) \cup \{ a \})$.
%
However, expressing $\widehat{\beta}$ as a linear combination of all actions $\cA(c)$ may be suboptimal if it leads to a significantly smaller set $\cC_\train$. For example, say $|\cA(c)| = 11$, and there is only one training context containing all of these actions, i.e., $|\cC(\cA(c) \cup \{ a \})| = 1$. Suppose there is a subset $\cA' \subset \cA(c)$, with $|\cA'| = 10$ with $|\cC(\cA' \cup \{ a \})| = 100$, i.e., by excluding a single action from the linear combination, we are able to train on 100 times more contexts.
%
Thus, we may consider the SI estimator induced by a specific \textit{donor set} $\cA_\donor \subseteq \cA(c)$, with the corresponding set of training contexts being $\cC_\train = \cC(\cA_\donor \cup \{ a \} )$.
%
The choice of donor set introduces a tradeoff: as the number of donor actions increases, the number of training contexts might decrease. This raises the question of how to pick an optimal set of donor actions for a given prediction.

{%\color{red}
\textbf{Picking donor actions.}
The subspace inclusion hypothesis test introduced in \rref{sec:subspace-test} suggests an elegant method for picking a set of donor actions: for a fixed significance level, find a set passing the hypothesis test which \textit{maximizes} the number of training contexts. 
%
Unfortunately, this induces a combinatorial optimization problem which may be difficult to solve when there are many actions. 
%
We consider two computationally efficient alternatives. 
%
First, we may greedily pick actions, according to whichever action \textit{least} reduces the number of training contexts, until the set passes the hypothesis test. 
%
Second, we may \textit{always} use $\cA(c)$ as the donor set, then use the subspace inclusion hypothesis test described above to decide on whether to use the SI estimate.
}%Even this method would incur high computational overhead, since each evaluation of the test statistic requires an SVD. }

% We implement simplified version of the above criteria -- we always use $\cA(c)$, but before prediction, we test whether it satisfies the hypothesis test or not. And based on that, we decide whether to trust the predictions or not. 
%In the following section, we found that picking the largest possible valid set of donor actions performed well, and thus did not attempt to optimize the donor set.


%Consider the task of imputing $\bx^{ca}$ for a target context $c$ and target action $a$. 
 

%For every $a \notin \Ac(c)$, 



==> content/setup.tex <==
\section{Problem Statement} \label{sec:problem_statement} 
We consider a collection of contexts (e.g., cell types), denoted by $\cC$, and actions (e.g., compounds or drugs), denoted
by $\cA$. The outcomes or measurements of interest associated with a given context $c \in \cC$ 
under action $a \in \cA$ are denoted by $\bx^{ca} \in \bbR^p$. Collectively, this forms an order-three
tensor $\mathcal{X} = [\bx^{ca}: c \in {\cC}, a \in {\cA}] \in \bbR^{|{\cC}| \times |{\cA}| \times p}$. 
%Our primary interest is in estimating $\mathcal{X}$.

%Towards this, we have access to limited observations corresponding to small number of experiments that are already conducted. 

{\bf Observations.} To model real-world scenarios, we consider the setup where we only have access to a sparse subset of the entries in $\mathcal{X}$ (e.g., corresponding to a limited number of historical experiments).  
%
Formally, let $\Omega \subset \cC \times \cA$ denote the context-action pairs for which
we observe their associated outcomes, i.e., for each $(c, a) \in \Omega$, we observe $\bx^{ca}$. 
%

{\bf Goal.} Our primary interest is in recovering $\mathcal{X}$ from $\Omega$. 

{\em Notations.}
%We define a few useful notations. Specifically, 
For any $a \in \cA$ and $c\in \cC$, let 
$\cA(c) = \{a \in \cA: (c, a) \in \Omega \}$ and $\cC(a) = \{c \in \cC: (c, a) \in \Omega \}$ denote the set of actions which are measured for context $c$, and the set of contexts which are measured for action $a$, respectively.
%
These notations are extended to sets of contexts and actions, i.e., $\cA(\cC) = \cap_{c \in \cC} \cA(c)$ and $\cC(\cA) = \cap_{a \in \cA} \cC(a)$. 

%Let ${\cC}$ and ${\cA}$ denote the collections of contexts and actions, respectively. 
%
%We define the tensor of \textit{outcomes} as $\mathcal{X} = [\bx^{ca}: c \in {\cC}, a \in {\cA}] \in \bbR^{|{\cC}| \times |{\cA}| \times p}$, where $\bx^{ca} \in \bbR^p$ denotes the outcome vector associated with context $c$ under action $a$. 
%The goal is to determine $\mathcal{X}$. 

%
% To formalize the SI estimator (and its modification) in the causal imputation setup, we now introduce some notation. Let $\bx^{ca} \in \bbR^p$ denote the \textit{outcome} vector associated with context $c$ under action $a$. 
%
%To that end, we discuss observations. Let $\Av_a(c)$ denote the \emph{available or observed actions} 
%for context $c$, i.e., $a \in \Av_a(c)$ if and only if $\bx^{ca}$ is measured. 
%%
%Similarly, let $\Av_c(a)$ denote the \emph{available or observed contexts} for action $a$. 
%
%These notations are extended to sets of contexts and actions, respectively, by requiring that outcomes 
%be available for all elements in the set, i.e., $\Av_a(\cC) = \cap_{c \in \cC} \Av_a(c)$ and 
%$\Av_c(\cA) = \cap_{a \in \cA} \Av_c(a)$.
